Studying the Impact of TensorFlow and PyTorch Bindings on Machine Learning Software Quality

Bindings for machine learning frameworks (such as TensorFlow and PyTorch) allow developers to integrate a framework's functionality using a programming language different from the framework's default language (usually Python). In this paper, we study the impact of using TensorFlow and PyTorch bindings in C#, Rust, Python and JavaScript on the software quality in terms of correctness (training and test accuracy) and time cost (training and inference time) when training and performing inference on five widely used deep learning models. Our experiments show that a model can be trained in one binding and used for inference in another binding for the same framework without losing accuracy. Our study is the first to show that using a non-default binding can help improve machine learning software quality from the time cost perspective compared to the default Python binding while still achieving the same level of correctness.

==> sections/motivation.tex <==
% \section{A Motivational Example}\label{sec:motivation}

% Anna's team uses JavaScript as the primary programming language. Since the team lacks ML or Python expertise, they collaborate with the company's ML team to integrate DL techniques into their projects. They are now considering using an ML framework's JavaScript binding for their project. However, they are concerned about how their developed ML software's quality is impacted by the binding; in particular, they are concerned about the correctness and time cost. 
% There are three possible scenarios for integration of the binding:
% % \begin{enumerate}[\textbf{-}]
% \begin{itemize}
%     \item \textbf{Integration Scenario 1:} The ML team develops and trains the DL models and ships the pre-trained models to Anna. In this scenario, Anna needs to use the JavaScript binding to load the pre-trained models and perform model inference in her project. %Anna is concerned about the the correctness and time cost of utilizing the binding for model inference.
%     \item \textbf{Integration Scenario 2:} The ML team assists Anna in training DL models in the project's native language which is JavaScript, allowing Anna to alter and maintain the code more efficiently. After training the DL models, Anna needs to deploy the trained models to the production environment in JavaScript as well. %Anna is concerned about the correctness and time cost of utilizing the binding for both model training and inference.
%     \item \textbf{Integration Scenario 3:} Since computational resources for the project are very limited, Anna is also open to a third scenario, in which the ML team assists her in selecting the most efficient combination of training and inference bindings in any language. In this scenario, Anna is willing to hire an expert in the chosen language(s) to help with the integration of the binding(s) as long as the reduction in computational resources is large enough.
% \end{itemize}
% % \end{enumerate}
% Our study results and our methodology can help Anna choose the best scenario.


